On fast bounded locality sensitive hashing

In this paper, we examine the hash functions expressed as scalar products, i.e., $f(x)=<v,x>$, for some bounded random vector $v$. Such hash functions have numerous applications, but often there is a need to optimize the choice of the distribution of $v$. In the present work, we focus on so-called anti-concentration bounds, i.e. the upper bounds of $\mathbb{P}\left[|<v,x>| < \alpha \right]$. In many applications, $v$ is a vector of independent random variables with standard normal distribution. In such case, the distribution of $<v,x>$ is also normal and it is easy to approximate $\mathbb{P}\left[|<v,x>| < \alpha \right]$. Here, we consider two bounded distributions in the context of the anti-concentration bounds. Particularly, we analyze $v$ being a random vector from the unit ball in $l_{\infty}$ and $v$ being a random vector from the unit sphere in $l_{2}$. We show optimal up to a constant anti-concentration measures for functions $f(x)=<v,x>$. As a consequence of our research, we obtain new best results for \newline \textit{$c$-approximate nearest neighbors without false negatives} for $l_p$ in high dimensional space for all $p\in[1,\infty]$, for $c=\Omega(\max\{\sqrt{d},d^{1/p}\})$. These results improve over those presented in [16]. Finally, our paper reports progress on answering the open problem by Pagh~[17], who considered the nearest neighbor search without false negatives for the Hamming distance.

==> circle_picture.tex <==
\begin{figure}[ht!]

\centering

\begin{tikzpicture}[scale = 0.3]

\draw[pattern=north east lines] (0,0) circle (2cm);
\draw[dashed] (0,0) circle (3cm);
\draw(0,0) circle (7cm);


\begin{scope}[rotate=315]
    \draw[thick,->] (0,0) -- (2,0) node[anchor=west] {$R$};
\end{scope}
\begin{scope}[rotate=345]
    \draw[thick,->] (0,0) -- (3,0) node[anchor=west] {$\sqrt{\log{\log{d}}} R$};
\end{scope}

\begin{scope}[rotate=285]
    \draw[thick,->] (0,0) -- (7,0) node[anchor=west] {$c R$};
\end{scope}

\node[align=left] at (0,0)   {$q$ \;\;};
\node at (1,1)   {\textbullet $p_1$};
\node at (2,4)   {\textbullet $p_3$};
\node at (-1,-2) {\textbullet $p_2$};
\node at (-7,4) {\textbullet $p_4$};


\end{tikzpicture}
\caption{The presented algorithms guarantee that points in the dashed area ($p_1$) will be reported as neighbors.
    Points within the dotted circle ($p_2$) will be reported as neighbor with high probability.
    Points ($p_3$) within a distance $cR$  might be reported, but not necessarily.
    Points ($p_4$) outside circle $cR$ cannot be reported. 
    }
\label{fig:circle}
\end{figure}

